Causality is all you need

In the fundamental statistics course, students are taught to remember the well-known saying: "Correlation is not Causation". Till now, statistics (i.e., correlation) have developed various successful frameworks, such as Transformer and Pre-training large-scale models, which have stacked multiple parallel self-attention blocks to imitate a wide range of tasks. However, in the causation community, how to build an integrated causal framework still remains an untouched domain despite its excellent intervention capabilities. In this paper, we propose the Causal Graph Routing (CGR) framework, an integrated causal scheme relying entirely on the intervention mechanisms to reveal the cause-effect forces hidden in data. Specifically, CGR is composed of a stack of causal layers. Each layer includes a set of parallel deconfounding blocks from different causal graphs. We combine these blocks via the concept of the proposed sufficient cause, which allows the model to dynamically select the suitable deconfounding methods in each layer. CGR is implemented as the stacked networks, integrating no confounder, back-door adjustment, front-door adjustment, and probability of sufficient cause. We evaluate this framework on two classical tasks of CV and NLP. Experiments show CGR can surpass the current state-of-the-art methods on both Visual Question Answer and Long Document Classification tasks. In particular, CGR has great potential in building the "causal" pre-training large-scale model that effectively generalizes to diverse tasks. It will improve the machines' comprehension of causal relationships within a broader semantic space.

==> parts/application_old.tex <==
\subsection{Application to our Model}

\noindent \textbf{Visual Question Answering (Computer Vision Task).}  In VQA task, X represents the multimodal input set composed of the image and question (i.e., RoI image features and language features learned through the language encoder). Z represents question-attended visual regions and attributes. Y represents the predicted answer. For direct effect modeling, we use the classic multimodal Transformer model called MCAN (Deep Modular Co-Attention Network).

For back-door adjustment, we select the observable confounding factor Z' as the question-guided common scene related to the visual RoI entities. As illustrated in the example given in Fig.\ref{fig:draft}, there is a prominent visual region "banana", and the question is ``what color is the banana?". The intuitively correct answer might be ``yellow" because "Banana has the property of yellow" is a common and relevant scene for the current question. Therefore, we determine that Z' has the following characteristics: 
\begin{itemize}
    \item Z' associates the prominent visual regions with the key question entities.
    \item Z' represents the common scene of these entities.
    \item Z' is detached from specific image context but influenced by the given question.
\end{itemize}

Fortunately, with the support of existing external knowledge resources, we can determine observable instances of Z' for each input image-question pair. ConceptNet integrates common relationships between numerous entity concepts in the form of knowledge triplets, and each triplet is accompanied by a statistical weight indicating the reliability of the information source. The higher the statistical weight when more information sources confirm the veracity of the current knowledge triplet. Therefore, we adopt the statistical weight as a measure of the commonness of the scene described by the current knowledge triplet. We determine Z' based on the following steps:

\begin{itemize}
    \item \textbf{Determining query keywords}: We define the following types of textual data as query keywords: (1) image object labels; (2) OCR text extraction results from the image; (3) n-gram entity phrases in the question. We choose image object labels and OCR results because they represent the semantic information of the key visual regions in the image, without involving global scene information, which satisfies the requirements of Z' characteristic 1 and 3. Additionally, we apply phrase part-of-speech restrictions to filter out crucial entity information.
    \item \textbf{Retrieval and Evaluation}: Based on the keywords determined in Step 1, we retrieve relevant knowledge triplets from ConceptNet. Considering the requirements of Z' features 2 and 3, we need to select knowledge triplets that not only align with the question requirements but are also more commonly observed. Therefore, we assign scores to each triplet. Firstly, we transform the triplets into knowledge sentences using templates based on the relationship type. For example, the knowledge triplet $\langle$\#subj\#, relatedTo, \#obj\#$\rangle$ is transformed into ``subj is related to obj". Subsequently, we utilize a pre-trained language model (in this paper, MPNet is used) to encode the question text and all the knowledge sentences. We calculate the cosine similarity between the two sets of encoding vectors as a measure of semantic consistency between the knowledge triplets and the question information.
    \begin{equation}
    \begin{split}
        [\alpha_Q]_i = \frac{s_Q\cdot [s_K]_i}{|s_Q|\cdot |[s_K]_i|}
    \end{split}  
    \label{eq:back-door eval}
    \end{equation}
    Where $s_Q$ and $[s_K]_i$ represent the encoding vectors of the question and the i-th knowledge sentence, respectively. Finally, we multiply the semantic consistency by the corresponding statistical weight of the knowledge triplet as the Z' score.
\end{itemize}

We select the top-M knowledge sentences as the Z' observations for each image-question pair.

\noindent \textbf{Long Document Classification (Natural Language Processing Task).} In LDC task, X represents the input document collection, Z represents several key information extracted from long documents used for classification, and Y represents the classification results. For direct effect modeling, we adopt a hierarchical Transformer model as the base long-sequence model.

For backdoor adjustment, we select the top-m words based on TF-IDF values in each long document as observable confounding Z', because the classification results should be influenced by the specific contextual information of the document, while these words possess frequency-based information instead of contextual information, which means they are most likely to mislead the classification results. 

==> parts/methodology_old.tex <==
\subsubsection{Causal Routing Architecture}

Causal Routing aims to explore the dominant causal relationships at different levels of hierarchical reasoning models. Therefore, we choose the Transformer model with a stacked structure of attention layers as the backbone network for Causal Routing. The Transformer model consists of an encoder and a decoder, both composed of multiple stacked encoding or decoding layers. The encoding layers are responsible for information integration, while the decoding layers handle information interaction and reasoning. As shown in Fig.\ref{fig:causal routing}, we equip the Transformer with multiple causal modules, namely Causal Transformer Blocks, each implementing a causal intervention for attention. An intuitive solution to identify the dominant causal modules is to assign weights to the outputs of Causal Transformer Blocks in each decoding layer and use a weighted sum as the output of the current decoding layer. Naturally, to obtain the final output of the Transformer decoder, we assign weights to the outputs of each decoding layer and compute the weighted sum of all decoding layer outputs.

Specifically, assuming a Transformer model with L decoding layers, each layer consisting of B Causal Transformer Blocks, the output of the Transformer decoder is obtained by:
\begin{equation}
\begin{split}
    C_l &= \sum_{b=1}^{B} C_{l,b} * [f^{norm}_C([W_C]_l)]_{l, b} \\
    X &= \sum_{l=1}^{L}C_l * [f^{norm}_L([W_L])]_l
\end{split}  
\label{eq:causal routing arch}
\end{equation}
Where $C_{l,b}$ represents the output of the b-th Causal Transformer Block in the l-th decoding layer, $f^{norm}_{\{C,L\}}$ denotes the normalization function for the causal block-level and layer-level weights (to be described in the next section), $W_C$ is the weight matrix for the outputs of the causal block-level, $C_l$ is the output of the l-th decoding layer, $W_L$ is the weight vector for the outputs of the layer-level, and $X$ represents the final output of the decoder. We set both $W_C$ and $W_L$ as learnable parameters, initialized with equal constants, indicating that the routing weight learning starts without any prior bias towards a specific causal block or decoding layer output.

\subsubsection{Selection Process}

By using the softmax function in equation (1) as the implementation of $f^{norm}_{\{C,L\}}$, we obtain continuous and differentiable weight values, enabling the dynamic fusion of the outputs from the causal block-level and layer-level. We refer to this selection method as soft selection. The differentiability of soft selection ensures that the Transformer model can be directly optimized by the loss function, making the Causal Transformer equipped with soft selection easy to train without the need for additional hyperparameters.

If we want to learn explicit causal hierarchical chains in the Transformer instead of dynamically fusing based on weights, we need to perform a row-wise argmax operation on the learnable weights $W_C$ and $W_L$. However, this operation is not differentiable, preventing the model from being trained through back-propagation. Moreover, using soft selection during training and directly applying the argmax operation on $W_C$ and $W_L$ during testing would result in a significant discrepancy in attention fusion features between training and testing. 

Therefore, we refer to the Gumbel softmax trick, which allows for discrete sampling from a probability distribution. We remove the noise term Gumbel(0, 1) from the Gumbel softmax function, making the output of $f^{norm}_{\{C,L\}}$ stable and closer to one-hot normalized weights. We refer to this improved softmax function as the \textit{sharpening softmax} function, which is defined as follows:
\begin{equation}
\begin{split}
    [f^{norm}(\alpha)]_i = \frac{exp(log(\alpha_i) / \tau)}{\sum_j exp(log(\alpha_j) / \tau)}
\end{split}  
\label{eq:selection process}
\end{equation}
where $\alpha$ represents the normalized weights after softmax, while $\tau$ denotes the temperature coefficient for sharpening the softmax function. At the initial stage of training, $\tau$ is set to 1, making the sharpening softmax function equivalent to the softmax function. As the training progresses, $\tau$ gradually decreases, and when $\tau$ converges to 0, the sharpening softmax function becomes more similar to the argmax function. By introducing the sharpening softmax function, we can optimize the weight matrix $[W_C]$ at the causal block level and the weight vector $[W_L]$ at the layer level using back-propagation, and make these weights approach the one-hot distribution more closely after training.

\subsection{Causal Routing Transformer for VQA}

In this work, we develop a Causal Routing Transformer for the task of Visual Question Answering (VQA). We illustrate the concepts of a) Direct Effect, b) Back-door Adjustment, and c) Front-door Adjustment in the context of VQA as follows:

\subsubsection{Direct Causal Effect}

We assume that the VQA task is free from confounding, as the causal relationship between the input and output is unaffected. We can design a model that directly predicts P(Y|X). In this case, we model the direct causal effect using the classic multimodal Transformer model called MCAN (Deep Modular Co-Attention Network). The direct causal graph, as shown in the Causal Graph section of Figure 2, represents the relationship between X, Z, and Y. Here, X represents the multimodal input set composed of the image and question (i.e., RoI image features and language features learned through the language encoder). Z represents specific visual regions and their attributes that are attended to based on the question. Y represents the predicted answer.

Thus, X→Z indicates that the attention mechanism in the MCAN decoder selects several RoI regions as candidate knowledge for answering the question based on the question features. Z→Y indicates that the reasoning system predicts the answer Y based on the selected visual attributes. The optimization objective of MCAN is to capture this direct causal effect.
\begin{equation}
\begin{split}
    P(Y|X)=\sum_{z}P(Y|Z=z)P(Z=z|X)
\end{split}  
\label{eq:direct}
\end{equation}
where z represents the visual and linguistic attributes from each selected RoI region.

\subsubsection{Back-Door Adjustment}

We assume that there exists an observable confounding factor Z' that influences the relationship between the input X and the output Y. Z provides a shortcut from X to Y, such as an implicit statistical relationship between the input and labels (for a given input sample x, most cases correspond to a specific output y, and the remaining output types Y' occur rarely, indicating an accumulation of incorrect shortcuts based on superficial input-label pairs). It misleads the model to deviate from the specific input examples and establishes erroneous dependencies. Since the confounding element Z' is observable, we can block the X→Z'→Y pathway through the backdoor adjustment principle, denoted as $P(Y|do(X))$, where $do(\cdot)$represents the intervention operation. 
\begin{equation}
\begin{split}
    P(Y|do(X))=\sum_{z\in Z'}P(Z'=z)\sum_{X=x}P(Y|X=x, Z'=z)
\end{split}  
\label{eq:back-door}
\end{equation}
where $z$ represents each instance of the observable confounding factor Z'.

In the VQA task, we select the observable confounding factor Z' as the question-guided common scene related to the visual RoI entities. As illustrated in the example given in Fig.\ref{fig:draft}, there is a prominent visual region "banana" in the image, and the question is "what color is the banana?". The intuitively correct answer might be "yellow" because "Banana has the property of yellow" is a common and relevant scene for the current question. Therefore, we determine that Z' has the following characteristics: 
\begin{itemize}
    \item Z' associates the prominent visual regions with the key entities in the question.
    \item Z' represents the common scene information of these entity concepts.
    \item Z' is detached from specific image context but influenced by the specific question information.
\end{itemize}

Fortunately, with the support of existing external knowledge resources, we can determine observable instances of Z' for each input image-question pair. ConceptNet integrates common relationships between numerous entity concepts in the form of knowledge triplets, and each triplet is accompanied by a statistical weight indicating the reliability of the information source. The higher the statistical weight when more information sources confirm the veracity of the current knowledge triplet. Therefore, we adopt the statistical weight as a measure of the commonness of the scene described by the current knowledge triplet. We determine Z' based on the following steps:

\begin{itemize}
    \item \textbf{Determining query keywords}: We define the following types of textual data as query keywords: (1) image object labels; (2) OCR text extraction results from the image; (3) n-gram entity phrases in the question. We choose image object labels and OCR results because they represent the semantic information of the key visual regions in the image, without involving global scene information, which satisfies the requirements of Z' characteristic 1 and 3. Additionally, we apply phrase part-of-speech restrictions to filter out crucial entity information.
    \item \textbf{Retrieval and Evaluation}: Based on the keywords determined in Step 1, we retrieve relevant knowledge triplets from ConceptNet. Considering the requirements of Z' features 2 and 3, we need to select knowledge triplets that not only align with the question requirements but are also more commonly observed. Therefore, we assign scores to each triplet. Firstly, we transform the triplets into knowledge sentences using templates based on the relationship type. For example, the knowledge triplet <subj, Related To, obj> is transformed into "subj is related to obj". Subsequently, we utilize a pre-trained language model (in this paper, MPNet is used) to encode the question text and all the knowledge sentences. We calculate the cosine similarity between the two sets of encoding vectors as a measure of semantic consistency between the knowledge triplets and the question information.
    \begin{equation}
    \begin{split}
        [\alpha_Q]_i = \frac{s_Q\cdot [s_K]_i}{|s_Q|\cdot |[s_K]_i|}
    \end{split}  
    \label{eq:back-door eval}
    \end{equation}
    Where $s_Q$ and $[s_K]_i$ represent the encoding vectors of the question and the i-th knowledge sentence, respectively. Finally, we multiply the semantic consistency by the corresponding statistical weight of the knowledge triplet as the Z' score.
\end{itemize}

We select the top-M knowledge sentences as the Z' observations for each image-question pair.

\subsubsection{Front-Door Adjustment}

We assume that there exists an unobservable confounding factor Z' that affects the relationship between the input X and the output Y, such as biases introduced by imbalanced data distributions, resulting in reduced model sensitivity to certain rare but significant inputs. An appropriate causal pathway should be consistent with the direct effect in a) (i.e., X→Z→Y), but the confounding factor Z' introduces a backdoor path Z←X←Z’→Y. 

In the VQA task, there are often frequent co-occurrences of certain concepts in the dataset, which can mislead the attention system to focus on the wrong visual regions. For example, in Fig.\ref{fig:draft}, the co-occurrence frequency of "sport" and "man" is much higher than that of "sport" and "screen". These confounding factors hidden in the data are difficult to observe, so we use the front-door adjustment principle for intervention. Specifically, we calculate the average causal effect of Z on Y to block the link X→Z.
\begin{equation}
\begin{split}
    P(Y|do(Z))=\sum_{x}P(X=x)P(Y|X=x,Z)
\end{split}  
\label{eq:front-door 1}
\end{equation}

By substituting $P(Y|do(Z))$ for $P(Y|Z=z)$ in the estimation of the direct causal effect, we can obtain the estimate of the true causal effect through front-door adjustment:
\begin{equation}
\begin{split}
    P(Y|do(X))&=\\
    \sum_{z}P(Y|&Z=z)\sum_{x}P(X=x)P(Y|X=x,Z=z)
\end{split}  
\label{eq:front-door 2}
\end{equation}


\subsection{Network Structure}

The Causal Transformer Block we constructed is illustrated in Fig.\ref{fig:causal block}. We implement the Causal Transformer Block for the direct causal effect using the Guided-Attention module of MCAN. The Causal Transformer Block consists of a Language Encoder and a Vision Decoder. For the implementation of Front-Door Adjustment, we follow the settings of IS \& CS-Sampling in CATT. We additionally input sentence dictionaries to the language encoder and image dictionaries to the decoder to reduce spurious correlations caused by frequent co-occurrence of entity concepts. Moreover, the Dict Cross-ATT module shares the parameters of the Self-ATT module in the MCAN backbone used for the direct causal effect to ensure that the outputs remain in the same space. For the implementation of Back-Door Adjustment, we adopt cross-attention. In the decoder part, we input the observed values of Z' as additional input. Each block stacks two Knowledge Cross-ATT modules, where the query is the observed value of Z', and the key and value are the image features and language features, respectively.

==> parts/methodology_old_2.tex <==
\input{plots/plot_cgr_layer}
\input{plots/plot_cgr_block}

\subsection{Stack Causal Networks}
\label{subsec: stak cn}

In this section, we illustrate how to implement our CGR architecture in a deep framework. 
In practice, we adopt the stacked networks to perform the causal routing computation, integrating direct effect, back-door adjustment, front-door adjustment, and probability of sufficient cause.

% In this section, we illustrate the implementation details of each causal intervention network, including the computation of block-level intra-layer causal sufficiency probabilities and fusion weights for inter-layer outputs. We adopt the Transformer as the hierarchical backbone network to implement the Causal Routing strategy. In the subsequent sub-sections, we will introduce how to modify the attention layer to achieve the three classic causal interventions mentioned above.

\subsubsection{Block of Direct Effect}

This block involves two stages: 1) extract the mediator M from the input X ($X \rightarrow M$) and 2) predict the outcome Y based on M ($M \rightarrow Y$). We have: 
% \noindent \textbf{Direct Effect.} The direct causal effect is the prediction approach adopted by most models. This process consists of two stages: extracting key attributes Z based on input X ($X\rightarrow Z$) and predicting the outcome Y based on the key attributes Z ($Z\rightarrow Y$).
\begin{equation}
\begin{split}
    P(Y|X)=\sum_{m}P(M=m|X)P(Y|M=m)
\end{split}  
\label{eq:direct prob}
\end{equation}
% Considering that most models output classification probabilities, we convert the aforementioned probabilistic formula into a network parameter description as follows: input X is passed through an aggregation embedding network $f_D^{emb}(X)$ to extract the key attributes Z, and then passed through the inference network $f_D^{inf}(X,Z)$ to obtain the hidden state, and finally the probability output $P(Y|X)$ is produced through the softmax function.
Considering that most CV tasks are formulated as classification problems, we compute $P(Y|X)$ using a transform function $f_D^{trans}$ and a multi-layer perceptron layer $MLP(\cdot )$. The former aims to extract the mediator $M$ from the input $X$, while the latter outputs classification probabilities through the softmax layer. 
{\color{blue}{\begin{equation}
\begin{split}
    E_X(M)&=f_D^{trans}(X)\\
    P(Y|X)&=softmax(MLP(E_X(M)))
\end{split}  
\label{eq:direct network}
\end{equation}}}
% \begin{equation}
% \begin{split}
%     &P(Y|Z=z):\quad P(Y|X)=softmax(f_D^{inf} (X, \hat{Z}))\\
%     &P(Z=z|X):\quad \hat{Z}=f_D^{emb}(X)\\
%     &\qquad \qquad \qquad \qquad=\sum_{X=x}P(X=x|f_{D(X\rightarrow \hat{Z})}^{emb}(X))x
% \end{split}  
% \label{eq:direct network}
% \end{equation}
% where the function $f_{D(X\rightarrow Z)}^{emb}(X)$ represents an embedding network applied to the input X, which maps the input X to a query space for producing the key features Z. In the framework of stacked causal networks, both X and Z are sets of embedding vectors that can be packed into matrix form.

% We employ the classical attention layer as the implementation approach for direct effect. The computation process of the attention layer aligns with the above formalized prediction process of direct effect, which selects the key features Z from the input X through self-attention or cross-attention and utilizes them in the subsequent reasoning process as follows:
% We employ the classical attention layer as the implementation approach. The computation process of the attention layer aligns with the above formalized prediction process, which selects the key features M from the input X and utilizes them for prediction:
% \begin{equation}
% \begin{split}
%     Q_D=f_{D_q}(X)\quad &K_D=f_{D_k}(X)\quad V_D=f_{D_v}(X)\\
%     A_D&=softmax(Q_D^T K_D)\\
%     M&=A_D V_D
% \end{split}  
% \label{eq:direct att}
% \end{equation}
% where $f_{D_q}$, $f_{D_k}$, and $f_{D_v}$ represent the query, key, and value embedding functions of the input X, respectively. Each attention vector in $A_D$ is a probability estimation $P(Z=z|X)$.

{\color{blue}{We use the classical attention layer $Attention(Q,K,V)\\=softmax(\frac{Q^T K}{\sqrt{d}})V$  to calculate 
$f^{trans}_D(X) = Attention(X,X,X)$. The queries $Q$, keys $K$ and values $V$ come from the input $X$. $d$ is the dimension of queries and keys. As shown in Fig. X(a), in the $l$-th layer, we take the result of $MLP(Ex(M))$ as the output of the direct effect block $C^{(l)}_{do_0}$. }}

% We use the classical attention layer to calculate both $f^{trans}_D(\cdot )$ and $f^{pre}_D(\cdot )$ as: 
% \begin{equation}
% \begin{split}
%     A_D&=softmax(\frac{Q_D^T K_D}{\sqrt{d}})\\
%     M&=A_D V_D
% \end{split}  
% \label{eq:direct att}
% \end{equation}
% In this case, all of queries $Q_D$, keys $K_D$ and values $V_D$ come from the same input $X$. 
% $d$ is the dimension of queries and keys.  
% Each attention vector in $A_D$ is a probability estimation $P(M = m|X)$. 
% where $f_{D_q}$, $f_{D_k}$, and $f_{D_v}$ represent the query, key, and value embedding functions of the input X, respectively, and $d$ is the dimension of input $X$. Each attention vector in $A_D$ is a probability estimation $P(Z=z|X)$.

% \noindent \textbf{Back-door Adjustment.} We assume that an observable confounding factor $Z$ influences the relationship between input X and output Y. We block the $X\rightarrow Z\rightarrow Y$ pathway through the backdoor adjustment, denoted as $P(Y|do(X))$:
\subsubsection{Block of Back-door Adjustment}
We assume that an observable confounder $Z$ influences the relationship between input X and output Y. 
The link $Z\rightarrow X$ is blocked through the backdoor adjustment, and then the causal effect of $X$ on $Y$ is identifiable and given by
(the detailed derivations are presented in supplementary material)
\begin{equation}
\begin{split}
    P(Y|do_1(X))=\sum_{z\in Z}P(Z=z)[P(Y|X, Z=z)]
\end{split}  
\label{eq:back-door}
\end{equation}
% \begin{equation}
% \begin{split}
%     P(Y&|do_1(X))=\\
%     &\sum_{X=x}\sum_{z\in Z}P(Z=z)[P(Y|X=x, Z=z)]
% \end{split}  
% \label{eq:back-door}
% \end{equation}
% where $do(\cdot)$ represents the intervention operation. In order to implement backdoor intervention in the network, we need to sample X and Z. Here, we use Normalized Weighted Geometric Mean to incorporate external sampling into the feature representation. Specifically, using the NWGM approximation, we can convert the probability formula in Eq.\ref{eq:back-door} into a network representation.
% where $do(\cdot)$ represents the intervention operation. To implement $P(Y|do(X))$, We need to sample X and Z and feed them into the network. Producing the expectation for all sampled values can be computationally expensive. Therefore, we employ the Normalized Weighted Geometric Mean (NWGM) to incorporate the outer sampling into the feature representation as an approximation of the sampling results. We denote the expectation for input X as \textbf{input estimation} and the expectation for the observable confounder Z as \textbf{confounding estimation}.
where $X$ and $Z$ denotes the embedding of inputs and confounders, respectively. To perform the back-door intervention operation, we parameterize $P(Y| X,Z)$ using a network, which final layer is a softmax function as: 
\begin{equation}
\begin{split}
    P(Y | X, Z = z) = softmax( f^{pre}_B( X, Z ) ) 
\end{split}  
\label{eq:back-door network}
\end{equation}
where $f^{pre}_B(\cdot )$ is the fully connected layer predictor. 
However, it requires an extensive amount of $X$ and $Z$ sampled from this network in order to compute $P(Y|do_1(X))$. 
We employ the Normalized Weighted Geometric Mean (NWGM) [][] to approximate the expectation of the softmax as the softmax of the expectation: 
{\color{blue}{\begin{equation}
\begin{split}
P(Y|do_1(X))&=E_{Z}(softmax(f^{pre}_B (X,Z)) \\
&\approx softmax(f^{pre}_B (E_{X}(X), E_{X}(Z)))
\end{split}  
\label{eq:back-door network}
\end{equation}}}
We calculate two query sets from $X$ and $Z$ to estimate the input expectation $E_{z}(X)$ and the confounder expectation $E_{z}(Z)$, respectively, as: 
{\color{blue}{\begin{equation}
\begin{split}
    E_{X}(X)&=\sum_{X=x}P(X=x|f_{B(X\rightarrow E_{X}(X))}^{emb}(X))x\\
    E_{X}(Z)&=\sum_{X=x}P(Z=z|f_{B(X, Z \rightarrow E_{X}(Z))}^{emb}(X))x
\end{split}  
\label{eq:back-door network}
\end{equation}}}
where $f_{B(X\rightarrow E_{X}(X))}^{emb}$ and $f_{B(X, Z \rightarrow E_{X}(Z))}^{emb}$ denote query embedding functions. 
% \begin{equation}
% \begin{split}
%     P(Y|do_1(X))&\approx softmax(f^{inf}_B(\hat{X}, \hat{Z}))\\
%     \hat{X}&=\sum_{Z=z}P(X=x|f_{B(X\rightarrow \hat{X})}^{emb}(X))z\\
%     \hat{Z}&=\sum_{Z=z}P(X=x|f_{B(X, Z \rightarrow \hat{Z})}^{emb}(Z))z
% \end{split}  
% \label{eq:back-door network}
% \end{equation}
% where $f_{B(X\rightarrow \hat{X})}^{emb}$ and $f_{B(X, Z \rightarrow \hat{Z})}^{emb}$ respectively represent the embedding networks for input estimation and confounding estimation, while $f^{inf}_B$ represents the output network for back-door adjustment. The derivation details of Eq.\ref{eq:back-door network} are provided in the supplementary material.
% We denote the computation of the sample estimate $\hat{X}$ from input X as an \textbf{intra-sample estimation}, and the computation of the confounding estimate $\hat{Z}$ from inputs X and observable confounder Z as an \textbf{intra-sample confounding estimation}. In Eq.\ref{eq:back-door network}, $f_{B(X\rightarrow \hat{X})}^{emb}$ and $f_{B(X, Z \rightarrow \hat{Z})}^{emb}$ respectively represent the embedding networks for intra-sample estimation and intra-sample confounding estimation, while $f^{inf}_B$ represents the output network for back-door adjustment. The derivation details of Eq.\ref{eq:back-door network} are provided in the supplementary material.

{\color{blue}{As shown in Fig. X(b), we use the classical attention layer to estimate the expectations of both variables: $E_X(X) = Attention(X,X,X)$ and $E_X(Z) = Attention(Z,X,X)$. In the $l$-th layer, both of them are concatenated and passed through a multi-layer perceptron layer to produce the output of the back-door block $C^{(l)}_{do_1}$.}}

% {\color{blue}{For the estimation $\hat{X}$, we adopt a self-attention layer. For the estimation $\hat{Z}$, we employ cross-attention layer.
% \begin{equation}
% \begin{split}
%     A_B&=softmax(\frac{Q_B^T K_B}{\sqrt{d}})\\
%     \hat{Z}&=A_B V_B
% \end{split}  
% \label{eq:back-door att}
% \end{equation}
% where $Q_B$ is generated from $Z$, and $K_B$ and $V_B$ are generated from $X$.}}
% \begin{equation}
% \begin{split}
%     Q_B=f_{B_q}(Z)\quad &K_B=f_{B_k}(X)\quad V_B=f_{B_v}(X)\\
%     A_B&=softmax(Q_B^T K_B)\\
%     \hat{Z}&=A_B V_B
% \end{split}  
% \label{eq:back-door att}
% \end{equation}
% where the query set is generated from $\hat{Z}$, and $f_{B_q}$ represents the query embedding network. $K_B$ and $V_B$ are generated from $\hat{X}$, $f_{B_k}$ and $f_{B_v}$ represent the embedding networks for the key set and value set, respectively.

\subsubsection{Block of Front-door Adjustment}

% \noindent \textbf{Front-door Adjustment.} We assume that there exists an unobservable confounding factor $Z$ that affects the relationship between the input X and the output Y. An appropriate causal pathway should be consistent with the Direct Effect (i.e., $X\rightarrow Z\rightarrow Y$), but the confounding factor Z introduces a backdoor path $Z\leftarrow X\leftarrow Z’\rightarrow Y$. Specifically, we calculate the average causal effect of Z on Y to block the link $X\rightarrow Z$.
We assume that an unobservable confounder $Z$ influences the relationship between input $X$ and output $Y$, while an observable mediator $M$ establishes a connection from $X$ to $Y$. We block the link $M\rightarrow Y$ through the front-door adjustment, and the causal effect of $X$ on $Y$ is given by (the detailed derivations are given in supplementary material) 
% \begin{equation}
% \begin{split}
%     P(Y|do_2(Z))=\sum_{x}P(X=x)P(Y|X=x,Z)
% \end{split}  
% \label{eq:front-door 1}
% \end{equation}

% By substituting $P(Y|do(Z))$ for $P(Y|Z=z)$ in the estimation of the direct causal effect, we can obtain the estimate of the true causal effect through front-door adjustment:
\begin{equation}
\begin{split}
    P(Y|do_2(X))&=\\
    \sum_{M=m}P(Y|&M=m)\sum_{x}P(X=x)P(Y|X=x,M=m)
\end{split}  
\label{eq:front-door 2}
\end{equation}
where X and M denotes the embedding of inputs and mediators, respectively. 
Similar to the back-door adjustment, we parameterize $P(Y| X=x, M=m)$ using the softmax-aware network and the Normalized Weighted Geometric Mean (NWGM) approximation. We have: 
% We adopted the front-door adjustment approach, employing the NWGM approximation to incorporate the estimates of input X and mediator Z into the feature layer.
{\color{blue}{\begin{equation}
\begin{split}
    % P(Y|do(X))&\approx softmax(f^{inf}_F(\hat{X}, \hat{Z}))\\
    P(Y |do_2(X)) &\approx softmax( f^{pre}_F( E_{X}(X), E_{X}(M) ) )
\end{split}  
\label{eq:front-door network}
\end{equation}}}
where $f^{pre}_F(\cdot )$ is the fully connected layer. 
Similarly, we estimate the expectations of variables by two query embedding functions $f_{F(X\rightarrow \hat{X})}^{emb}$ and $f_{F(X \rightarrow \hat{Z})}^{emb}$. 
{\color{blue}{\begin{equation}
\begin{split}
    % P(Y|do(X))&\approx softmax(f^{inf}_F(\hat{X}, \hat{Z}))\\
    E_X(X)&=\sum_{X=x}P(X=x|f_{F(X\rightarrow E_X(X))}^{emb}(X))x\\
    E_X(M)&=\sum_{M=m}P(M=m|f_{F(X \rightarrow E_X(M))}^{emb}(X))m
\end{split}  
\label{eq:front-door network}
\end{equation}}}
% where $f_{F(X\rightarrow \hat{X})}^{emb}$ and $f_{F(X \rightarrow \hat{Z})}^{emb}$ represent the transformation network of input X into two query sets.

{\color{blue}{Similarly, we employ the classical attention layer to estimate the expectations, denoted as $E_X(X) = Attention(X,D_X,D_X)$ and $E_X(M) = Attention(X,X,X)$. Different from the above two blocks, we utilize the global dictionary $D_X$, which is initialized by conducting K-means clustering on all the sample features of the training dataset, to generate keys and values. In the $l$-th layer, the concatenated expectations are fed into a multi-layer perceptron to generate the output of the front-door block $C^{(l)}_{do_2}$. }}

% {\color{blue}{For the estimation $\hat{M}$, we employ a classical attention layer. As for the estimated value $\hat{X}$, we utilize global dictionary from the training dataset to generate key and value set.
% \begin{equation}
% \begin{split}
%     A_F&=softmax(\frac{Q_F^T K_F}{\sqrt{d}})\\
%     \hat{X}&=A_F V_F
% \end{split}  
% \label{eq:back-door att}
% \end{equation}
% where $Q_F$ comes from input $X$, $K_F$ and $V_F$ are generated from global dictionary.}}

% \begin{equation}
% \begin{split}
%     A_F&=softmax(\frac{f_{F_q}(X)^T f_{F_k}(Dict_X))}{\sqrt{d}}\\
%     \hat{X}&=A_F f_{F_v}(Dict_X)
% \end{split}  
% \label{eq:back-door att}
% \end{equation}
% \begin{equation}
% \begin{split}
%     Q_F=f_{F_q}(X)\quad &K_F=f_{F_k}(Dict_X)\quad V_F=f_{F_v}(Dict_X)\\
%     A_F&=softmax(Q_F^T K_F)\\
%     \hat{X}&=A_F V_F
% \end{split}  
% \label{eq:back-door att}
% \end{equation}
% where $f_{F_q}$ denotes query embedding network for input X, $f_{F_k}$ and $f_{F_v}$ represent the embedding networks for the key set and value set generated from global dictionary.

\input{plots/plot_cgr_arch}

\subsubsection{Probability of Sufficient Cause}

In our architecture, each layer consists of three deconfounding modules from different causal graphs. 
We reexamine Eq. 3, and find that the process of evaluating the total effect $P(Y|do(X))$ is essentially to search the optimal deconfounding graph among three causal graphs, while the other two causal graphs are sufficient causal conditions for the optimal solution. 
For example, 
during the game of building blocks, if we discover that both graph B and C are ineffective, it naturally leads to use the graph A as the optimal building method. 
Take $TE_{P_1} = P_1(y|do_1{x}) *( ps_{P_2\rightarrow P_1} + ps_{P_3\rightarrow P_1} )$ an example. 
When both $ps_{P_2\rightarrow P_1}$ and $ps_{P_3\rightarrow P_1}$ have high values, indicating that both $P_2$ and $P_3$ are sufficient cause for $P_1$, we consider $P_1$ as the optimal deconfounding method for achieving $P(Y|do(X))$. 
Therefore, in this paper, we calculate the weight of the causal graph $P_1$ to approximate the probability of sufficient cause where $P_1$ is the optimal solution. 
Similarly, we calculate the weight of the causal graph $P_2$ to approximate the probability of $P_2$ being the optimal solution. 
We have: 
\begin{equation}
\begin{split}
C^{(l)} =   \sum^B_{b=1}  f^{norm}( w^{(l)} )  * C^{(l)}_b
\end{split}  
\label{eq:causal weight 1}
\end{equation}
where $w^{(l)}$ is the weight vector of the l-th layer. Its each element $w^{(l)}_i {i=1,2,3}$ reflects the probability of the i-th causal block as the optimal solution of the l-th layer. 
$f^{norm}(\cdot)$ denotes the normalization function (described in Optimization). 
$C^{(l)}_b$ represents the output of the b-th causal block in the l-th layer. 
$C^{(l)}$ is the output of the l-th causal layer. 
In this work, we employ L = 6 parallel causal layers and combine them as: 
\begin{equation}
\begin{split}
C =  \sum^L_{l=1}  f^{norm}( w^{(c)} )  * C^{(l)}
\end{split}
\label{eq:causal weight 2}
\end{equation}
where $w^{(c)}$ is the layer-aware weight vector. $C$ represents the final output, which is computed as a weighted sum of all causal layers. 
Both $w^{(l)}$ and $w^{(c)}$ are learnable parameters, initialized with equal constants, indicating that the routing weight learning starts without any prior bias towards a specific causal block or layer. 

\noindent \textbf{Optimization.}
To enable the dynamic fusion of causal blocks and causal layers, we design the sharpening softmax function to implement $f^{norm}(\cdot )$. 
Particularly, we remove the noise term $Gumbel (0,1)$ from the Gumbel softmax function as: 
\begin{equation}
\begin{split}
    [f^{norm}(\alpha)]_i = \frac{exp(log(\alpha_i) / \tau)}{\sum_j exp(log(\alpha_j) / \tau)}
\end{split}  
\label{eq:selection process}
\end{equation}
where $\alpha$ represents the normalized weight vector after softmax; $\alpha_i$ is the $i$-th weight value; $\tau$ denotes the temperature coefficient for sharpening the softmax function. At the initial stage of training, the value of $\tau$ is set to 1, which results in the sharpening softmax function being the same as the regular softmax function. As the training progresses, $\tau$ gradually decreases, and as it converges to 0, the sharpening softmax function starts to resemble the argmax function more closely. By the designed sharpening softmax function, the block- and layer-aware weight vectors can be optimized through back-propagation. This optimization process enhances the performance of these weights, resulting in more noticeable differences after training. 

% \subsubsection{Selection Process}
% \label{subsubsec: sel pro}

% By using the softmax function in equation (1) as the implementation of $f^{norm}$, we obtain continuous and differentiable weights, enabling the dynamic fusion of the block-level and layer-level outputs. We refer to this selection method as soft selection. The differentiability of soft selection ensures that the CGR model can be directly optimized by the loss function.

% However, the weights generated by the softmax function do not have a clear differentiation. In order to make the normalization function produce a sharper distribution, we remove the noise term Gumbel(0, 1) from the Gumbel softmax function, and name this function as \textit{sharpening softmax} function:
% \begin{equation}
% \begin{split}
%     [f^{norm}(\alpha)]_i = \frac{exp(log(\alpha_i) / \tau)}{\sum_j exp(log(\alpha_j) / \tau)}
% \end{split}  
% \label{eq:selection process}
% \end{equation}
% where $\alpha$ represents the normalized weights after softmax, $\tau$ denotes the temperature coefficient for sharpening the softmax function. At the initial stage of training, $\tau$ is set to 1, making the sharpening softmax function equivalent to the softmax function. As the training progresses, $\tau$ gradually decreases, and when $\tau$ converges to 0, the sharpening softmax function becomes more similar to the argmax function. By introducing the sharpening softmax function, we can optimize the block-level weight matrix $[W_C]$ and the layer-level weight vector $[W_L]$ using back-propagation, and make these weights perform more significant differences after training.

% \subsubsection{Causal Weights}

% As shown in Fig.\ref{fig:causal routing}, we equip the Transformer with multiple causal network blocks, each implementing a causal intervention for attention. An intuitive solution to identify the dominant causal modules is to assign block-level weights for intra-layer outputs and layer-level weights for inter-layer outputs. Specifically, assuming a Causal Routing Transformer with L layers, each layer consisting of B causal network blocks, the output is produced by:
% \begin{equation}
% \begin{split}
%     C_l &= \sum_{b=1}^{B} C_{l,b} * [f^{norm}_C([W_C]_l)]_{l, b} \\
%     C &= \sum_{l=1}^{L}C_l * [f^{norm}_L([W_L])]_l
% \end{split}  
% \label{eq:causal routing arch}
% \end{equation}
% where $C_{l,b}$ represents the output of the b-th causal network block in the l-th layer, $f^{norm}_{\{C,L\}}$ denotes the normalization function for the causal block-level and layer-level weights (to be described in the next section), $W_C$ is the block-level weight matrix, $C_l$ is the output of the l-th decoding layer, $W_L$ is the layer-level weight vector, and $C$ represents the final output. We set both $W_C$ and $W_L$ as learnable parameters, initialized with equal constants, indicating that the routing weight learning starts without any prior bias towards a specific causal block or layer output.

% \subsubsection{Selection Process}

% By using the softmax function in equation (1) as the implementation of $f^{norm}_{\{C,L\}}$, we obtain continuous and differentiable weight values, enabling the dynamic fusion of the outputs from the causal block-level and layer-level. We refer to this selection method as soft selection. The differentiability of soft selection ensures that the Causal Routing Transformer can be directly optimized by the loss function.

% If we want to learn explicit causal hierarchical chains instead of dynamically fusing, we need to perform a row-wise argmax operation on the learnable weights $W_C$ and $W_L$. However, this operation is not differentiable, preventing the model from being trained through back-propagation. Moreover, using soft selection during training and directly applying the argmax operation on $W_C$ and $W_L$ during testing would result in a significant discrepancy in attention fusion features between training and testing. 

% Therefore, we refer to the Gumbel softmax trick, which allows for discrete sampling from a probability distribution. We remove the noise term Gumbel(0, 1) from the Gumbel softmax function, making the output of $f^{norm}_{\{C,L\}}$ stable and sharp. We refer to this improved softmax function as the \textit{sharpening softmax} function:
% \begin{equation}
% \begin{split}
%     [f^{norm}(\alpha)]_i = \frac{exp(log(\alpha_i) / \tau)}{\sum_j exp(log(\alpha_j) / \tau)}
% \end{split}  
% \label{eq:selection process}
% \end{equation}
% where $\alpha$ represents the normalized weights after softmax, while $\tau$ denotes the temperature coefficient for sharpening the softmax function. At the initial stage of training, $\tau$ is set to 1, making the sharpening softmax function equivalent to the softmax function. As the training progresses, $\tau$ gradually decreases, and when $\tau$ converges to 0, the sharpening softmax function becomes more similar to the argmax function. Therefore, we can make $[W_C]$ and $[W_L]$ exhibit a relatively distinct internal difference.

\input{parts/application}

